DEMix Layers: Disentangling Domains for Modular Language Modeling

We introduce a new domain expert mixture (DEMix) layer that enables conditioning a language model (LM) on the domain of the input text. A DEMix layer is a collection of expert feedforward networks, each specialized to a domain, that makes the LM modular: experts can be mixed, added or removed after initial training. Extensive experiments with autoregressive transformer LMs (up to 1.3B parameters) show that DEMix layers reduce test-time perplexity, increase training efficiency, and enable rapid adaptation with little overhead. We show that mixing experts during inference, using a parameter-free weighted ensemble, allows the model to better generalize to heterogeneous or unseen domains. We also show that experts can be added to iteratively incorporate new domains without forgetting older ones, and that experts can be removed to restrict access to unwanted domains, without additional training. Overall, these results demonstrate benefits of explicitly conditioning on textual domains during language modeling.

==> tables/balancing_domains.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t]
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rccc}
\toprule
& \multicolumn{3}{c}{\bf \gptthree}\\
& SM & MD & LG \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-4}
\bf \dataparallel  & 20.5 & 16.5 & 14.5 \\
\bf \dataparallel (Balanced) & \bf 19.9 & \bf 16.0 & \bf 14.3 \\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

\bottomrule
\end{tabular}

% }
\caption{Average of in-domain test-set perplexity, across three model sizes. Balancing domain exposure during training improves in-domain performance, especially for domains that are less prevalent (e.g. \oneb, \reviews, and \cs). See Appendix for a per-domain breakdown of these results. } 
\label{tab:balancing_results}
\end{table}


==> tables/dapt.tex <==
% \begin{table*}[t]\small
% \centering
% % \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% &  \multicolumn{4}{c}{ \bf GPT-3 Small} \\
% \cmidrule{2-5}
% % % \emph{Shared Params}  & 124M & 124M & 96.1M & 67.8M  \\
% % % \emph{Expert Params}  & 0 & 0 & 28.3M & 56.7M  \\
% % % \emph{Total Params} & 124M & 124M & 322.8M & 521.1M  \\
% % \cmidrule{2-5}

% \textbf{Domain} & \bf \dataparallel  & \bf \domaintoken & \bf \plusmodelayers (L/2) & \bf \plusmodelayers (L) \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% \midrule 

% \oneb 


% % 82.1
% & 14.6 & 14.2 & 14.3 & \bf 13.5  \\ %& 79.0$_{4.1}$\\


% \cs 
% % 82.1
% & 17.9 & 17.8 & 17.0 & \bf 15.6  \\ %& 79.0$_{4.1}$\\


% \legal 
% % 82.1
% & 10.5 & 10.1 &  9.5 & \bf 9.0   \\ %& 79.0$_{4.1}$\\


% \med  
% % 82.1
% & 13.8 & 14.1 & 13.4 & \bf 11.8 \\ %& 79.0$_{4.1}$\\


% \webtext 
% % 82.1
% & 22.0 & \bf 20.5 & 21.8 & 21.1 \\%& 79.0$_{4.1}$\\


% \realnews 
% % 82.1
% & 20.1 & \bf 18.6 & 20.0 &  18.8 \\ %& 79.0$_{4.1}$\\


% \reddit 
% % 82.1
% & 40.9 & \bf 40.3 & 41.6 &  40.8 \\ %& 79.0$_{4.1}$\\


% \reviews 
% % 82.1
% & 23.9 &  23.2 & 22.3 &  \bf 20.5\\ %& 79.0$_{4.1}$\\

% \midrule
% \bf Average & 20.5 & 19.9 &  20.0 & \bf 18.9 \\

% \bottomrule
% \end{tabular}
% % }
% \caption{Conditioning GPT-3 small on domains improves in-domain test performance, when training with 32 GPUs for 48 hours. See Appendix \label{sec:validation_curves} for validation curves during training.} 
% \label{tab:base_results}
% \end{table*}


\begin{table}[t] \small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rccc}
\toprule
&  \multicolumn{3}{c}{\bf Parameters}\\
& 125M & 350M & 760M \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-4}
\bf \dense & 23.3 & 19.0 & 16.5 \\
\bf \demix & 19.6 & 16.5 & 15.7 \\
\cmidrule{2-4}
\bf \densedapt & 42.9 & 17.8 & 15.4 \\
\bf \demixdapt & \bf 16.9 & \bf 14.3 & \bf 13.6 \\


% \cmidrule{3-5}
% \parbox[t]{0.7}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{In-Domain}}}}} & \bf \dense  & 20.6 & 16.5 & 14.5 \\
% & \bf \densedapt & 69.0 & 21.0 & 17.4 \\
% & \bf \demix (estimated prior) & \bf 17.8 & \bf 14.7 & \bf 13.9 \\
% & \bf \demixdapt & 17.7 & 14.6 & 13.7 \\
% \cmidrule{3-5}
% \parbox[t]{0.7}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{Out-of-Domain}}}}} & \bf \dense   & 25.9 & 21.4 & 18.4 \\
% & \bf \densedapt  & 16.7 & 14.6 & 13.3 \\
% & \bf \demix (estimated prior) & \bf 21.4 & \bf 18.3 & \bf 17.4 \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% & \bf \demixdapt & 16.0 & 14.0 & 13.5 \\
%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

\bottomrule
\end{tabular}

% }
\caption{Global average between in-domain and out-of-domain test-set perplexity before and after \dapt, across three model sizes.} 
\label{tab:dapt_results}
\end{table}


==> tables/data_scaling.tex <==
\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rccc}
\toprule
& \multicolumn{3}{c}{\bf \gptthree Small}\\
& 32 GPUs & 64 GPUs & 128 GPUs \\
% \bf \multicolumn{1}{p{0.5cm}}{\centering Model \\ (GPUs)} &  \multicolumn{1}{p{0.5cm}}{\centering SM \\ (32)}  &  \multicolumn{1}{p{0.5cm}}{\centering SM \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering SM \\ (128)} \\
\cmidrule{2-4}
\bf \dataparallel  & 19.9  & X & X \\
\bf \modelayers & 19.0 & X & X\\ %& \boldmath{\lnot}\textbf{\dapt}\\
\bf $\Delta$ & --0.9 & X & X\\ %& \boldmath{\lnot}\textbf{\dapt}\\

\bottomrule
\end{tabular}

% }
\caption{Given a fixed model size, \modelayers make progressively better use of increased computational budgets than \dataparallel.} 
\label{tab:data_scaling}
\end{table}

==> tables/efficiency_results.tex <==
\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
& \multicolumn{4}{c}{\bf \gptthree}\\
\bf \multicolumn{1}{p{0.5cm}}{\centering Model \\ (GPUs)} &  \multicolumn{1}{p{0.5cm}}{\centering SM \\ (32)}  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-4}
\bf \dataparallel & X & X & X   \\
\bf \gshard & X & X & X   \\
\bf \domainparallel  & X  & X & X  \\
\bottomrule
\end{tabular}

% }
\caption{\domainparallel is more efficient than \gshard. We measure efficiency in updates per second} 
\label{tab:efficiency_results}
\end{table}

==> tables/improving_indomain.tex <==


\begin{table}[t]
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rccc}
\toprule
& \multicolumn{3}{c}{\bf \gptthree}\\
& SM & MD & LG \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-4}
\bf \dataparallel  & 19.9 & 16.0 & 14.3 \\
\bf \domaintoken & 19.2 & 16.0 & 14.3 \\
\bf \shortdemixlayers &  19.0 & 15.5 & 14.1\\ %& \boldmath{\lnot}\textbf{\dapt}\\
\bottomrule
\end{tabular}

% }
\caption{Mixing experts also improves in-domain results significantly. See Appendix \label{sec:validation_curves} for validation curves during training.} 
\label{tab:improving_indomain}
\end{table}


==> tables/moe_comparison.tex <==
\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rccc}
\toprule
& \multicolumn{3}{c}{\bf \gptthree}\\
& SM & MD & LG \\
% \bf \multicolumn{1}{p{0.5cm}}{\centering Model \\ (GPUs)} &  \multicolumn{1}{p{0.5cm}}{\centering SM \\ (32)}  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)}\\
 \cmidrule{2-4}
\bf \shortmodelayers & 17.6  & 14.7 & 13.9 \\
\bf \gshard  & X & X & X  \\
\bottomrule
\end{tabular}


\begin{tabular}{rccc}
\toprule
& \multicolumn{3}{c}{\bf \gptthree}\\
& SM & MD & LG \\
% \bf \multicolumn{1}{p{0.5cm}}{\centering Model \\ (GPUs)} &  \multicolumn{1}{p{0.5cm}}{\centering SM \\ (32)}  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)}\\
 \cmidrule{2-4}
\bf \shortmodelayers (up/s)  & 1.27  & 0.59 & 0.36 \\
\bf \gshard (up/s) & 0.55 & 0.22 & X  \\
\bottomrule
\end{tabular}

% }
\caption {Domain parallel outperforms \gshard given the same computational budget \textbf{(top)}, while being more computationally efficient due to less GPU communication \textbf{(bottom)}. We measure efficency in number of updates per second. See Appendix \label{sec:validation_curves} for validation curves during training.} 
\label{tab:moe_comparison}
\end{table}

==> tables/ood_datasets.tex <==




\begin{table*}[t!]
\centering
\small
%  \resizebox{\textwidth}{!}{
\begin{tabular}{rlr}
\toprule
\bf Domain & \bf  Corpus & \bf \# Train (Eval) Tokens \\
\midrule

\gutenberg      
& 3.2M copyright-expired books \citep{gutenberg} & 3B (10M) \\
% \midrule[0.03em]
\textsc{Tweets}$^\dagger$ 
& 1M English tweets from 2013-2018 & 8M (1M)
\\

\cord 
& 400K COVID-19 Research Papers \citep{wang2020cord19} &  60M (10M) \\

\textsc{Github}
& 230K public Github repository contents  \citep{githubcode} & 200M (10M) \\

\textsc{Breaking News}$^\dagger$ 
& 20K latest articles from 400 English newspapers \citep{baly:2018:EMNLP2018}  & 11M (1M) \\


\textsc{Yelp Reviews}$^\dagger$ 
& 6M Yelp restaurant reviews \citep{yelpreviews} & 600M (10M)\\

\textsc{Contracts}$^\dagger$ & 500 commercial legal contracts \citep{hendrycks2021cuad} & 1.5M (1M) \\

\aclpapers & 1.5K ACL Papers from the Qasper dataset \citep{Dasigi2021ADO} & 1M (1M)  \\
\bottomrule
\end{tabular}
% }
\caption{Corpora for out-of-domain evaluation, including the size of our training and evaluation (i.e., validation and test) data, in whitespace-separated tokens. $\dagger$ indicates datasets that we (partially) anonymize (\S\ref{sec:dataset}).}
\label{tab:ood_datasets}
\end{table*}

==> tables/ood_removal.tex <==
\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
&  \multicolumn{3}{c}{ \bf 125M Parameters} \\





% Gutenberg Books	12.57%	9.69%
% Github Code	1.09%	16.59%
% Tweets	3.58%	9.81%
% CORD-19	29.00%	11.82%
% Breaking News	6.82%	30.83%
% Yelp Reviews	11.71%	3.30%
% Legal Contracts	10.66%	29.81%
% ACL Papers	34.44%	8.98%
% 	13.95%	13.78%




\cmidrule{2-4}

\textbf{Domain}  & \bf \demix & \bf --1 & \bf --2  \\
& \bf PPL & \bf\textsc{Expert} & \bf \textsc{Experts}  \\
%& \boldmath{\lnot}\textbf{\dapt}\\
\midrule 

\gutenberg 


% 82.1
& 33.4 & \bf	+12.6\% &  +9.7\%  \\ %& 79.0$_{4.1}$\\


\cord 
% 82.1
&  15.6 &	\bf +29.0\% &  +11.9\%   \\ %of  79.0$_{4.1}$\\


\github 
% 82.1
& 10.9	& +1.1\% &  \bf +16.6\%    \\ %& 79.0$_{4.1}$\\


\yelp  
% 82.1
 & 28.5 &	 \bf +11.7\% &  +3.3\%    \\ %& 79.0$_{4.1}$\\


\breakingnews 
% 82.1
 &  20.8 &	 +6.82\% & \bf +30.8\%   \\%& 79.0$_{4.1}$\\


\contracts 
% 82.1
& 10.8 &	+10.7\% &  \bf +29.8\%   \\ %& 79.0$_{4.1}$\\


\aclpapers 
% 82.1
 & 16.4 & \bf	+34.4\% &  +9.0\%   \\ %& 79.0$_{4.1}$\\


\tweets 
% 82.1
& 35.0 &	+3.6\% & \bf +9.8\%  \\ %& 79.0$_{4.1}$\\

\midrule
\bf Average &  21.4 & 	+13.7\% & \bf +15.1\%  \\

\bottomrule
\end{tabular}
% }
\caption{Given a novel domain, we remove the top 1, top 2, most likely experts according to the \demix model, each resulting in progressively worse zero-shot performance. Here, we display the rates of perplexity increase after each removal. We observe that domains have different rates of performance degradation with each expert removal; some domains only need one expert removed to see a large performance hit, while others need more experts removed. We bold the greatest rate of increase for each domain.}
\label{tab:ood_removal}
\end{table}

==> tables/scale_results.tex <==
\begin{table}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
& \multicolumn{3}{c}{\bf \gptthree}\\
\bf \multicolumn{1}{p{0.5cm}}{\centering Model \\ (GPUs)} &  \multicolumn{1}{p{0.5cm}}{\centering SM \\ (32)}  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-4}
\bf \dataparallel  & 19.9 & 16.0 & 14.3 \\
\bf \domaintoken & 19.2 & 16.0 & 14.3 \\
\bf \plusdomainparallel & 19.0 & 15.5 & 14.1\\ %& \boldmath{\lnot}\textbf{\dapt}\\
\bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

\bottomrule
\end{tabular}

% }
\caption{Average of in-domain performance at multiple scales. See Appendix \label{sec:validation_curves} for validation curves during training.} 
\label{tab:scale_results}
\end{table}

==> tables/shared_results.tex <==
\begin{table*}[t]\small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcc|cccc}
\toprule
\emph{Shared Params} & 70.4M & 70.4M & 57.8M & 70.4M & 70.4M \\
\emph{Expert Params} & 0 & 0.0 & 12.6M & 12.6M & 12.6M \\
\emph{Total Params} & 70.4M & 70.4M & 158.6M & 171.2M & 171.2M \\
\cline{2-6}
\textbf{Domain} & \bf DP  & \bf + D-Token & \bf FFN Experts & \bf + Shared Experts & \bf + Unmarked Expert \\ %& \boldmath{\lnot}\textbf{\dapt}\\
\midrule 

\oneb 

% 82.1
& X & X &  X & X & X \\ %& 79.0$_{4.1}$\\


\cs 
% 82.1
& X & X &  X & X & X \\ %& 79.0$_{4.1}$\\


\legal 
% 82.1
& X & X &  X & X & X \\ %& 79.0$_{4.1}$\\


\med  
% 82.1
& X & X &  X & X & X \\ %& 79.0$_{4.1}$\\


\webtext 
% 82.1
& X & X &  X & X & X \\%& 79.0$_{4.1}$\\


\realnews 
% 82.1
& X & X &  X & X & X \\ %& 79.0$_{4.1}$\\


\reddit 
% 82.1
& X & X &  X & X & X \\ %& 79.0$_{4.1}$\\


\reviews 
% 82.1
& X & X &  X & X & X \\ %& 79.0$_{4.1}$\\


\bottomrule
\end{tabular}
% }
\caption{Adding shared parameters improves in-domain test performance, when training with 8 GPUs for 24 hours.} 
\label{tab:main}
\end{table*}

==> tables/sixteen_experts.tex <==
\begin{table}[t] \small
\centering
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{rccc}
\toprule
&  \multicolumn{3}{c}{\bf Parameters}\\
& 125M & 350M & 760M \\
% &  \multicolumn{1}{p{0.5cm}}{\centering SM }  &  \multicolumn{1}{p{0.5cm}}{\centering MD \\ (64)} &  \multicolumn{1}{p{0.5cm}}{\centering LG \\ (128)} \\
\cmidrule{2-4}
\bf \dense & 23.3 & 19.0 & 16.5 \\
\bf \demix & 19.6 & 16.5 & 15.7 \\
\cmidrule{2-4}
\bf \densedapt & 42.9 & 17.8 & 15.4 \\
\bf \demixdapt & \bf 16.9 & \bf 14.3 & \bf 13.6 \\


% \cmidrule{3-5}
% \parbox[t]{0.7}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{In-Domain}}}}} & \bf \dense  & 20.6 & 16.5 & 14.5 \\
% & \bf \densedapt & 69.0 & 21.0 & 17.4 \\
% & \bf \demix (estimated prior) & \bf 17.8 & \bf 14.7 & \bf 13.9 \\
% & \bf \demixdapt & 17.7 & 14.6 & 13.7 \\
% \cmidrule{3-5}
% \parbox[t]{0.7}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\bf {\textsc{Out-of-Domain}}}}} & \bf \dense   & 25.9 & 21.4 & 18.4 \\
% & \bf \densedapt  & 16.7 & 14.6 & 13.3 \\
% & \bf \demix (estimated prior) & \bf 21.4 & \bf 18.3 & \bf 17.4 \\ %& \boldmath{\lnot}\textbf{\dapt}\\
% & \bf \demixdapt & 16.0 & 14.0 & 13.5 \\
%& \boldmath{\lnot}\textbf{\dapt}\\

%&\boldmath{\lnot}\textbf{\dapt}\\
% \bf \plusdomainparallel (Mixed) & \bf 17.6 & \bf 14.7 & \bf 13.9 \\ %& \boldmath{\lnot}\textbf{\dapt}\\

\bottomrule
\end{tabular}

% }
\caption{Global average between in-domain and out-of-domain test-set perplexity before and after \dapt, across three model sizes.} 
\label{tab:dapt_results}
\end{table}

